Engineering Multilevel Graph Partitioning Algorithms

We present a multi-level graph partitioning algorithm using novel local improvement algorithms and global search strategies transferred from the multi-grid community. Local improvement algorithms are based max-flow min-cut computations and more localized FM searches. By combining these techniques, we obtain an algorithm that is fast on the one hand and on the other hand is able to improve the best known partitioning results for many inputs. For example, in Walshaw's well known benchmark tables we achieve 317 improvements for the tables 1%, 3% and 5% imbalance. Moreover, in 118 additional cases we have been able to reproduce the best cut in this benchmark.

==> comparisions/hugegraphs_compressed_from_csv_rel.tex <==
%\tiny
%\begin{tabular}{|r|rrr|rrr|rrr|rrr|rrr|rrr|rrr|rrr|}
%\hline
  %&  \multicolumn{3}{c}{KaFFPa Strong}  & \multicolumn{3}{c}{KaFFPa Eco}  & \multicolumn{3}{c}{KaFFPa Fast}  & \multicolumn{3}{c}{KaSPar Strong}& \multicolumn{3}{c}{KaPPa Strong}& \multicolumn{3}{c}{DiBaP}& \multicolumn{3}{c}{Scotch}& \multicolumn{3}{c|}{Metis}\\ 
  %\hline
%$k$  &  Best.     &     Avg.            &           $t$ &  Best.     &     Avg.            &           $t$   & Best.     &     Avg.            &           $t$   &Best.     &     Avg.            &           $t$ & Best.     &     Avg.            &           $t$ & Best.     &     Avg.            &           $t$ & Best.     &     Avg.            &           $t$ & Best.     &     Avg.            & $t$\\  
  %\hline
%2  & \numprint{3988}  & \numprint{4001}  & \numprint{22,68}  & \numprint{3,23} & \numprint{4,42} & \numprint{0,79} & \numprint{14,67} & \numprint{11,45} & \numprint{0,40} & \numprint{0,63} & \numprint{1,15}  & \numprint{24,94}  & \numprint{2,53} & \numprint{4,47} & \numprint{11,63} & \numprint{7,45} & \numprint{28,84} & \numprint{2,25}  & \numprint{6,27}  & \numprint{10,72} & \numprint{0,71} & \numprint{13,92} & \numprint{18,02} & \numprint{0,39} \\
%4  & \numprint{10467} & \numprint{10559} & \numprint{50,18}  & \numprint{3,93} & \numprint{3,88} & \numprint{1,42} & \numprint{13,66} & \numprint{20,58} & \numprint{0,43} & \numprint{0,77} & \numprint{0,48}  & \numprint{32,09}  & \numprint{4,52} & \numprint{5,77} & \numprint{19,76} & \numprint{6,36} & \numprint{7,41}  & \numprint{2,79}  & \numprint{8,30}   & \numprint{9,68}  & \numprint{1,53} & \numprint{13,75} & \numprint{17,01} & \numprint{0,40} \\
%8  & \numprint{19288} & \numprint{19553} & \numprint{76,39}  & \numprint{6,86} & \numprint{7,71} & \numprint{2,06} & \numprint{19,38} & \numprint{24,25} & \numprint{0,50} & \numprint{0,23} & \numprint{-0,24} & \numprint{44,11}  & \numprint{5,01} & \numprint{5,40}  & \numprint{25,46} & \numprint{8,77} & \numprint{9,71}  & \numprint{4,31}  & \numprint{10,90}  & \numprint{11,52} & \numprint{2,46} & \numprint{16,22} & \numprint{18,63} & \numprint{0,42} \\
%16 & \numprint{31474} & \numprint{31953} & \numprint{111,49} & \numprint{5,75} & \numprint{5,96} & \numprint{2,82} & \numprint{14,23} & \numprint{14,95} & \numprint{0,64} & \numprint{0,64} & \numprint{0,15}  & \numprint{65,43}  & \numprint{4,28} & \numprint{3,96} & \numprint{26,66} & \numprint{7,58} & \numprint{7,62}  & \numprint{7,19}  & \numprint{11,23} & \numprint{11,29} & \numprint{3,54} & \numprint{15,25} & \numprint{15,81} & \numprint{0,43} \\
%32 & \numprint{48195} & \numprint{48506} & \numprint{145,04} & \numprint{6,06} & \numprint{6,56} & \numprint{3,94} & \numprint{13,55} & \numprint{14,80} & \numprint{0,80} & \numprint{1,19} & \numprint{1,54}  & \numprint{94,42}  & \numprint{3,92} & \numprint{4,26} & \numprint{21,84} & \numprint{6,00} & \numprint{6,74}  & \numprint{12,14} & \numprint{11,27} & \numprint{11,99} & \numprint{4,75} & \numprint{13,43} & \numprint{14,29} & \numprint{0,46} \\
%64 & \numprint{69936} & \numprint{70363} & \numprint{199,84} & \numprint{5,73} & \numprint{6,11} & \numprint{5,09} & \numprint{12,32} & \numprint{12,71} & \numprint{1,03} & \numprint{2,24} & \numprint{2,36}  & \numprint{126,59} & \numprint{4,15} & \numprint{4,20}  & \numprint{16,44} & \numprint{6,02} & \numprint{6,13}  & \numprint{21,17} & \numprint{10,64} & \numprint{10,91} & \numprint{6,14} & \numprint{12,12} & \numprint{12,56} & \numprint{0,50} \\
        %\hline
   %&   \numprint{20986} &   \numprint{21172} &   \numprint{80.93} &  \numprint{22088}& \numprint{22393}& \numprint{2.25}& \numprint{23952} &\numprint{24742}&\numprint{0.60}&  \numprint{21185} &   \numprint{21364} &   \numprint{54.97} &   \numprint{21839} &   \numprint{22163} &   \numprint{19.56} & \numprint{22460}&\numprint{23461}& \numprint{6.07}&   \numprint{23033} &   \numprint{23505}  &   \numprint{2.56} &   \numprint{23945} &   \numprint{24568} & \numprint{0.44}\\
          %\hline
%\end{tabular}


\small
\begin{tabular}{|r|rrr|rrr|}
\hline
                             & \multicolumn{3}{c}{KaFFPa Strong} & \multicolumn{3}{c|}{KaFFPa Eco}\\
\hline
$k$                          & Best.                             & Avg.                                 & $t$               & Best.            & Avg.             & $t$             \\
\hline
2                            & \numprint{3988}                   & \numprint{4001}                      & \numprint{22,68}  & \numprint{3,23}  & \numprint{4,42}  & \numprint{0,79} \\
4                            & \numprint{10467}                  & \numprint{10559}                     & \numprint{50,18}  & \numprint{3,93}  & \numprint{3,88}  & \numprint{1,42} \\
8                            & \numprint{19288}                  & \numprint{19553}                     & \numprint{76,39}  & \numprint{6,86}  & \numprint{7,71}  & \numprint{2,06} \\
16                           & \numprint{31474}                  & \numprint{31953}                     & \numprint{111,49} & \numprint{5,75}  & \numprint{5,96}  & \numprint{2,82} \\
32                           & \numprint{48195}                  & \numprint{48506}                     & \numprint{145,04} & \numprint{6,06}  & \numprint{6,56}  & \numprint{3,94} \\
64                           & \numprint{69936}                  & \numprint{70363}                     & \numprint{199,84} & \numprint{5,73}  & \numprint{6,11}  & \numprint{5,09} \\
\hline
Avg.                         & \numprint{20986}                  & \numprint{21172}                     & \numprint{80.93}  & \numprint{22088} & \numprint{22393} & \numprint{2.25} \\
\hline
\hline
                             & \multicolumn{3}{c}{KaFFPa Fast}   & \multicolumn{3}{c|}{KaSPar Strong}\\
\hline
                             & Best.                             & Avg.                                 & $t$               & Best.            & Avg.             & $t$               \\
\hline
2                            & \numprint{14,67}                  & \numprint{11,45}                     & \numprint{0,40}   & \numprint{0,63}  & \numprint{1,15}  & \numprint{24,94}  \\
4                            & \numprint{13,66}                  & \numprint{20,58}                     & \numprint{0,43}   & \numprint{0,77}  & \numprint{0,48}  & \numprint{32,09}  \\
8                            & \numprint{19,38}                  & \numprint{24,25}                     & \numprint{0,50}   & \numprint{0,23}  & \numprint{-0,24} & \numprint{44,11}  \\
16                           & \numprint{14,23}                  & \numprint{14,95}                     & \numprint{0,64}   & \numprint{0,64}  & \numprint{0,15}  & \numprint{65,43}  \\
32                           & \numprint{13,55}                  & \numprint{14,80}                     & \numprint{0,80}   & \numprint{1,19}  & \numprint{1,54}  & \numprint{94,42}  \\
64                           & \numprint{12,32}                  & \numprint{12,71}                     & \numprint{1,03}   & \numprint{2,24}  & \numprint{2,36}  & \numprint{126,59} \\
\hline
Avg.                         & \numprint{23952}                  & \numprint{24742}                     & \numprint{0.60}   & \numprint{21185} & \numprint{21364} & \numprint{54.97}  \\

\hline
\hline
                             & \multicolumn{3}{c}{KaPPa Strong}  & \multicolumn{3}{c|}{DiBaP} \\
\hline
                             & Best.                             & Avg.                                 & $t$               & Best.            & Avg.             & $t$              \\
\hline
2                            & \numprint{2,53}                   & \numprint{4,47}                      & \numprint{11,63}  & \numprint{7,45}  & \numprint{28,84} & \numprint{2,25}  \\
4                            & \numprint{4,52}                   & \numprint{5,77}                      & \numprint{19,76}  & \numprint{6,36}  & \numprint{7,41}  & \numprint{2,79}  \\
8                            & \numprint{5,01}                   & \numprint{5,40}                      & \numprint{25,46}  & \numprint{8,77}  & \numprint{9,71}  & \numprint{4,31}  \\
16                           & \numprint{4,28}                   & \numprint{3,96}                      & \numprint{26,66}  & \numprint{7,58}  & \numprint{7,62}  & \numprint{7,19}  \\
32                           & \numprint{3,92}                   & \numprint{4,26}                      & \numprint{21,84}  & \numprint{6,00}  & \numprint{6,74}  & \numprint{12,14} \\
64                           & \numprint{4,15}                   & \numprint{4,20}                      & \numprint{16,44}  & \numprint{6,02}  & \numprint{6,13}  & \numprint{21,17} \\
\hline
Avg.                         & \numprint{21839}                  & \numprint{22163}                     & \numprint{19.56}  & \numprint{22460} & \numprint{23461} & \numprint{6.07}  \\
                
\hline
\hline
                             & \multicolumn{3}{c}{Scotch}        & \multicolumn{3}{c|}{Metis}\\
\hline
                                                                                                                                   
                             & Best.                             & Avg.                                 & $t$               & Best.            & Avg.             & $t$\\
\hline
                                                                                                                                   
2                            & \numprint{6,27}                   & \numprint{10,72}                     & \numprint{0,71}   & \numprint{13,92} & \numprint{18,02} & \numprint{0,39} \\
4                            & \numprint{8,30}                   & \numprint{9,68}                      & \numprint{1,53}   & \numprint{13,75} & \numprint{17,01} & \numprint{0,40} \\
8                            & \numprint{10,90}                  & \numprint{11,52}                     & \numprint{2,46}   & \numprint{16,22} & \numprint{18,63} & \numprint{0,42} \\
16                           & \numprint{11,23}                  & \numprint{11,29}                     & \numprint{3,54}   & \numprint{15,25} & \numprint{15,81} & \numprint{0,43} \\
32                           & \numprint{11,27}                  & \numprint{11,99}                     & \numprint{4,75}   & \numprint{13,43} & \numprint{14,29} & \numprint{0,46} \\
64                           & \numprint{10,64}                  & \numprint{10,91}                     & \numprint{6,14}   & \numprint{12,12} & \numprint{12,56} & \numprint{0,50} \\
\hline
Avg.                         & \numprint{23033}                  & \numprint{23505}                     & \numprint{2.56}   & \numprint{23945} & \numprint{24568} & \numprint{0.44}\\

\hline






\end{tabular}




==> fragmaster/_bestbalancedcut2_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=6cm
%
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{b1}{$b_1$}
\psfrag{b2}{$b_2$}
\psfrag{B}{$B$}
\psfrag{G}{$G$}
\psfrag{s}{$s$}
\psfrag{t}{$t$}


==> fragmaster/_bestbalancedcut_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=6cm
%
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{b1}{$b_1$}
\psfrag{b2}{$b_2$}
\psfrag{B}{$B$}
\psfrag{G}{$G$}
\psfrag{s}{$s$}
\psfrag{t}{$t$}


==> fragmaster/closedvertexset_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=6cm
%
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{s}{$s$}
\psfrag{t}{$t$}
\psfrag{x}{$x$}
\psfrag{u}{$u$}
\psfrag{v}{$v$}
\psfrag{w}{$w$}
\psfrag{y}{$y$}
\psfrag{z}{$z$}


==> fragmaster/flowsituation_after_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=6cm
%
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{s}{$s$}
\psfrag{t}{$t$}
\psfrag{d}{$\partial_r B$}
\psfrag{r}{$\delta_r$}
\psfrag{B}{$B$}
\psfrag{b1}{$b_1$}
\psfrag{b2}{$b_2$}


==> fragmaster/flowsituation_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=6cm
%
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{b1}{$b_1$}
\psfrag{b2}{$b_2$}
\psfrag{B}{$B$}
\psfrag{G}{$G$}
\psfrag{s}{\small$s$}
\psfrag{t}{\small$t$}
\psfrag{dbl}{\tiny$\partial_lB$}
\psfrag{dbr}{\tiny$\partial_rB$}
\psfrag{sdr}{\tiny$\delta_r$}
\psfrag{sdl}{\tiny$\delta_l$}




==> regression/speed_up_plot <==
%PDF-1.4
%âãÏÓ\r
1 0 obj
<<
/CreationDate (D:20110105154437)
/ModDate (D:20110105154437)
/Title (R Graphics Output)
/Producer (R 2.12.0)
/Creator (R)
>>
endobj
2 0 obj
<<
/Type /Catalog
/Pages 3 0 R
>>
endobj
5 0 obj
<<
/Type /Page
/Parent 3 0 R
/Contents 6 0 R
/Resources 4 0 R
>>
endobj
6 0 obj
<<
/Length 7 0 R
>>
stream
1 J 1 j q
Q q
0.000 0.000 0.000 RG
0.75 w
[] 0 d
1 J
1 j
10.00 M
59.04 54.40 m 59.04 287.73 l S
59.04 54.40 m 51.84 54.40 l S
59.04 132.18 m 51.84 132.18 l S
59.04 209.96 m 51.84 209.96 l S
59.04 287.73 m 51.84 287.73 l S
BT
0.000 0.000 0.000 rg
/F2 1 Tf 0.00 12.00 -12.00 0.00 41.76 46.90 Tm (0.0) Tj
ET
BT
/F2 1 Tf 0.00 12.00 -12.00 0.00 41.76 124.68 Tm (0.5) Tj
ET
BT
/F2 1 Tf 0.00 12.00 -12.00 0.00 41.76 202.46 Tm (1.0) Tj
ET
BT
/F2 1 Tf 0.00 12.00 -12.00 0.00 41.76 280.23 Tm (1.5) Tj
ET
59.04 43.20 m
473.76 43.20 l
473.76 345.60 l
59.04 345.60 l
59.04 43.20 l
S
Q q
BT
0.000 0.000 0.000 rg
/F2 1 Tf 0.00 12.00 -12.00 0.00 12.96 119.65 Tm [( Speedup r) 18 (elative to Kmetis )] TJ
ET
Q q
0.000 0.000 0.000 RG
0.75 w
[] 0 d
1 J
1 j
10.00 M
74.40 43.20 m 458.40 43.20 l S
74.40 43.20 m 74.40 36.00 l S
117.07 43.20 m 117.07 36.00 l S
159.73 43.20 m 159.73 36.00 l S
202.40 43.20 m 202.40 36.00 l S
245.07 43.20 m 245.07 36.00 l S
287.73 43.20 m 287.73 36.00 l S
330.40 43.20 m 330.40 36.00 l S
373.07 43.20 m 373.07 36.00 l S
415.73 43.20 m 415.73 36.00 l S
458.40 43.20 m 458.40 36.00 l S
BT
0.000 0.000 0.000 rg
/F2 1 Tf 12.00 0.00 -0.00 12.00 59.47 17.28 Tm [(r) 18 (gg15)] TJ
ET
BT
/F2 1 Tf 12.00 0.00 -0.00 12.00 102.13 17.28 Tm [(r) 18 (gg16)] TJ
ET
BT
/F2 1 Tf 12.00 0.00 -0.00 12.00 144.80 17.28 Tm [(r) 18 (gg17)] TJ
ET
BT
/F2 1 Tf 12.00 0.00 -0.00 12.00 187.47 17.28 Tm [(r) 18 (gg18)] TJ
ET
BT
/F2 1 Tf 12.00 0.00 -0.00 12.00 230.13 17.28 Tm [(r) 18 (gg19)] TJ
ET
BT
/F2 1 Tf 12.00 0.00 -0.00 12.00 272.80 17.28 Tm [(r) 18 (gg20)] TJ
ET
BT
/F2 1 Tf 12.00 0.00 -0.00 12.00 315.47 17.28 Tm [(r) 18 (gg21)] TJ
ET
BT
/F2 1 Tf 12.00 0.00 -0.00 12.00 358.13 17.28 Tm [(r) 18 (gg22)] TJ
ET
BT
/F2 1 Tf 12.00 0.00 -0.00 12.00 400.80 17.28 Tm [(r) 18 (gg23)] TJ
ET
BT
/F2 1 Tf 12.00 0.00 -0.00 12.00 443.47 17.28 Tm [(r) 18 (gg24)] TJ
ET
Q q 59.04 43.20 414.72 302.40 re W n
0.000 0.000 0.000 RG
2.25 w
[] 0 d
1 J
1 j
10.00 M
74.40 179.83 m
117.07 221.55 l
159.73 244.30 l
202.40 267.91 l
245.07 281.71 l
287.73 301.53 l
330.40 316.82 l
373.07 318.97 l
415.73 333.74 l
458.40 333.82 l
S
0.663 0.663 0.663 RG
74.40 124.56 m
117.07 141.51 l
159.73 139.92 l
202.40 134.29 l
245.07 126.88 l
287.73 126.29 l
330.40 116.88 l
373.07 107.10 l
415.73 102.70 l
458.40 97.41 l
S
0.745 0.745 0.745 RG
74.40 60.48 m
117.07 60.57 l
159.73 60.62 l
202.40 58.94 l
245.07 58.70 l
287.73 59.56 l
330.40 58.64 l
373.07 58.46 l
415.73 57.33 l
458.40 56.61 l
S
Q q
0.000 0.000 0.000 RG
0.75 w
[] 0 d
1 J
1 j
10.00 M
59.04 43.20 m
473.76 43.20 l
473.76 345.60 l
59.04 345.60 l
59.04 43.20 l
S
Q q 59.04 43.20 414.72 302.40 re W n
0.000 0.000 0.000 RG
0.75 w
[] 0 d
1 J
1 j
10.00 M
59.04 209.96 m 473.76 209.96 l S
0.000 0.000 0.000 rg
68.65 335.99 7.69 -6.41 re B
0.663 0.663 0.663 rg
68.65 323.17 7.69 -6.41 re B
0.745 0.745 0.745 rg
68.65 310.36 7.69 -6.41 re B
BT
0.000 0.000 0.000 rg
/F2 1 Tf 11.00 0.00 -0.00 11.00 85.95 328.98 Tm (KaFFPa-Fast) Tj
ET
BT
/F2 1 Tf 11.00 0.00 -0.00 11.00 85.95 316.16 Tm (KaFFPa-Eco) Tj
ET
BT
/F2 1 Tf 11.00 0.00 -0.00 11.00 85.95 303.35 Tm [(KaFFPa-Str) 18 (ong)] TJ
ET
Q
endstream
endobj
7 0 obj
3094
endobj
3 0 obj
<<
/Type /Pages
/Kids [
5 0 R
]
/Count 1
/MediaBox [0 0 504 360]
>>
endobj
4 0 obj
<<
/ProcSet [/PDF /Text]
/Font <</F2 9 0 R >>
/ExtGState << >>
>>
endobj
8 0 obj
<<
/Type /Encoding
/BaseEncoding /WinAnsiEncoding
/Differences [ 45/minus 96/quoteleft
144/dotlessi /grave /acute /circumflex /tilde /macron /breve /dotaccent
/dieresis /.notdef /ring /cedilla /.notdef /hungarumlaut /ogonek /caron /space]
>>
endobj
9 0 obj <<
/Type /Font
/Subtype /Type1
/Name /F2
/BaseFont /Palatino-Roman
/FirstChar 32 /LastChar 255 /Widths [
 250 278 371 500 500 840 778 278 333 333 389 606 250
 606 250 606 500 500 500 500 500 500 500 500 500 500 250 250
 606 606 606 444 747 778 611 709 774 611 556 763 832 337 333
 726 611 946 831 786 604 786 668 525 613 778 722 1000 667 667
 667 333 606 333 606 500 278 500 553 444 611 479 333 556 582
 291 234 556 291 883 582 546 601 560 395 424 326 603 565 834
 516 556 500 333 606 333 606 0 0 0 0 0 0 0 0
 0 0 0 0 0 0 0 0 0 287 333 333 333 333 333
 333 250 333 0 333 333 0 380 313 333 250 278 500 500 500
 500 606 500 333 747 333 500 606 333 747 333 400 606 300 300
 333 603 628 250 333 300 333 500 750 750 750 444 778 778 778
 778 778 778 944 709 611 611 611 611 337 337 337 337 774 831
 786 786 786 786 786 606 833 778 778 778 778 667 604 556 500
 500 500 500 500 500 758 444 479 479 479 479 287 287 287 287
 546 582 546 546 546 546 546 606 556 603 603 603 603 556 601
 556]
/FontDescriptor 10 0 R
/Encoding 8 0 R
>> endobj
10 0 obj <<
 /Type /FontDescriptor
 /FontName /Palatino-Roman
 /Flags 34
 /FontBBox [-166 -283 1021 927]
 /CapHeight 692
 /Ascent 726
 /Descent -281
 /ItalicAngle 0
 /XHeight 469
 /StemV 83
>>
endobj
xref
0 11
0000000000 65535 f 
0000000021 00000 n 
0000000164 00000 n 
0000003460 00000 n 
0000003543 00000 n 
0000000213 00000 n 
0000000293 00000 n 
0000003440 00000 n 
0000003624 00000 n 
0000003881 00000 n 
0000004919 00000 n 
trailer
<<
/Size 11
/Info 1 0 R
/Root 2 0 R
>>
startxref
5119
%%EOF


==> tables/eps_1_ws_scratch.tex <==
3elt &       \textbf{\numprint{89}} & \numprint{89} & \textbf{\numprint{199}} & \numprint{199} & \textbf{\numprint{342}} & \numprint{342} & \numprint{571} & \textbf{\numprint{569}} & \numprint{987} & \textbf{\numprint{969}} & \numprint{1595} & \textbf{\numprint{1564}} & 
add20 &       \numprint{678} & \textbf{\numprint{594}} & \numprint{1197} & \textbf{\numprint{1177}} & \numprint{1740} & \textbf{\numprint{1704}} & \numprint{2156} & \textbf{\numprint{2121}} & \textbf{\numprint{2565}} & \numprint{2687} & \textbf{\numprint{3071}} & \numprint{3236} & 
data &       \textbf{\numprint{188}} & \numprint{188} & \textbf{\numprint{378}} & \numprint{383} & \textbf{\numprint{659}} & \numprint{660} & \numprint{1170} & \textbf{\numprint{1162}} & \numprint{2002} & \textbf{\numprint{1865}} & \numprint{2954} & \textbf{\numprint{2885}} & 
uk &       \textbf{\numprint{19}} & \numprint{19} & \textbf{\numprint{40}} & \numprint{41} & \textbf{\numprint{82}} & \numprint{84} & \textbf{\numprint{150}} & \numprint{152} & \numprint{260} & \textbf{\numprint{258}} & \textbf{\numprint{431}} & \numprint{438} & 
add32 &       \textbf{\numprint{10}} & \numprint{10} & \textbf{\numprint{30}} & \numprint{33} & \textbf{\numprint{66}} & \numprint{66} & \textbf{\numprint{117}} & \numprint{117} & \textbf{\numprint{212}} & \numprint{212} & \numprint{498} & \textbf{\numprint{493}} & 
bcsstk33 &       \textbf{\numprint{10097}} & \numprint{10097} & \numprint{21556} & \textbf{\numprint{21508}} & \numprint{34183} & \textbf{\numprint{34178}} & \numprint{55447} & \textbf{\numprint{54860}} & \numprint{79324} & \textbf{\numprint{78132}} & \numprint{110656} & \textbf{\numprint{108505}} & 
whitaker3 &       \textbf{\numprint{126}} & \numprint{126} & \textbf{\numprint{380}} & \numprint{380} & \textbf{\numprint{655}} & \numprint{656} & \numprint{1105} & \textbf{\numprint{1093}} & \textbf{\numprint{1700}} & \numprint{1717} & \numprint{2588} & \textbf{\numprint{2567}} & 
crack &       \textbf{\numprint{183}} & \numprint{183} & \textbf{\numprint{362}} & \numprint{362} & \textbf{\numprint{677}} & \numprint{678} & \numprint{1109} & \textbf{\numprint{1092}} & \numprint{1720} & \textbf{\numprint{1707}} & \numprint{2620} & \textbf{\numprint{2566}} & 
wing_nodal &       \textbf{\numprint{1695}} & \numprint{1696} & \numprint{3576} & \textbf{\numprint{3572}} & \numprint{5445} & \textbf{\numprint{5443}} & \textbf{\numprint{8417}} & \numprint{8422} & \numprint{12129} & \textbf{\numprint{11980}} & \numprint{16332} & \textbf{\numprint{16134}} & 
fe_4elt2 &       \textbf{\numprint{130}} & \numprint{130} & \textbf{\numprint{349}} & \numprint{349} & \textbf{\numprint{605}} & \numprint{605} & \textbf{\numprint{1006}} & \numprint{1014} & \textbf{\numprint{1647}} & \numprint{1657} & \numprint{2575} & \textbf{\numprint{2537}} & 
vibrobox &       \numprint{11538} & \textbf{\numprint{10310}} & \textbf{\numprint{19155}} & \numprint{19199} & \numprint{24702} & \textbf{\numprint{24553}} & \numprint{34384} & \textbf{\numprint{32167}} & \numprint{42711} & \textbf{\numprint{41399}} & \numprint{49924} & \textbf{\numprint{49521}} & 
bcsstk29 &       \textbf{\numprint{2818}} & \numprint{2818} & \numprint{8070} & \textbf{\numprint{8035}} & \numprint{14291} & \textbf{\numprint{13965}} & \numprint{23280} & \textbf{\numprint{21768}} & \numprint{36125} & \textbf{\numprint{34886}} & \numprint{58613} & \textbf{\numprint{57054}} & 
4elt &       \textbf{\numprint{138}} & \numprint{138} & \textbf{\numprint{320}} & \numprint{321} & \textbf{\numprint{534}} & \numprint{534} & \textbf{\numprint{938}} & \numprint{939} & \numprint{1576} & \textbf{\numprint{1559}} & \numprint{2623} & \textbf{\numprint{2596}} & 
fe_sphere &       \textbf{\numprint{386}} & \numprint{386} & \textbf{\numprint{766}} & \numprint{768} & \textbf{\numprint{1152}} & \numprint{1152} & \textbf{\numprint{1710}} & \numprint{1730} & \textbf{\numprint{2520}} & \numprint{2565} & \numprint{3670} & \textbf{\numprint{3663}} & 
cti &       \textbf{\numprint{318}} & \numprint{318} & \textbf{\numprint{944}} & \numprint{944} & \textbf{\numprint{1752}} & \numprint{1802} & \textbf{\numprint{2865}} & \numprint{2906} & \textbf{\numprint{4180}} & \numprint{4223} & \numprint{6016} & \textbf{\numprint{5875}} & 
memplus &       \numprint{5596} & \textbf{\numprint{5489}} & \numprint{9805} & \textbf{\numprint{9559}} & \numprint{12126} & \textbf{\numprint{11785}} & \numprint{13564} & \textbf{\numprint{13241}} & \numprint{15232} & \textbf{\numprint{14395}} & \numprint{17595} & \textbf{\numprint{16857}} & 
cs4 &       \textbf{\numprint{366}} & \numprint{367} & \textbf{\numprint{938}} & \numprint{940} & \textbf{\numprint{1455}} & \numprint{1467} & \textbf{\numprint{2124}} & \numprint{2195} & \textbf{\numprint{2990}} & \numprint{3048} & \textbf{\numprint{4141}} & \numprint{4154} & 
bcsstk31 &       \textbf{\numprint{2699}} & \numprint{2701} & \textbf{\numprint{7296}} & \numprint{7444} & \textbf{\numprint{13274}} & \numprint{13371} & \numprint{24546} & \textbf{\numprint{24277}} & \numprint{38860} & \textbf{\numprint{38086}} & \numprint{60612} & \textbf{\numprint{60528}} & 
fe_pwt &       \textbf{\numprint{340}} & \numprint{340} & \textbf{\numprint{704}} & \numprint{704} & \textbf{\numprint{1437}} & \numprint{1441} & \textbf{\numprint{2799}} & \numprint{2806} & \textbf{\numprint{5552}} & \numprint{5612} & \textbf{\numprint{8314}} & \numprint{8454} & 
bcsstk32 &       \textbf{\numprint{4667}} & \numprint{4667} & \textbf{\numprint{9208}} & \numprint{9247} & \numprint{21253} & \textbf{\numprint{20855}} & \textbf{\numprint{36968}} & \numprint{37372} & \numprint{62994} & \textbf{\numprint{61144}} & \numprint{97299} & \textbf{\numprint{95199}} & 
fe_body &       \textbf{\numprint{262}} & \numprint{262} & \textbf{\numprint{598}} & \numprint{599} & \textbf{\numprint{1040}} & \numprint{1079} & \textbf{\numprint{1806}} & \numprint{1858} & \textbf{\numprint{2968}} & \numprint{3202} & \textbf{\numprint{5057}} & \numprint{5282} & 
t60k &       \textbf{\numprint{75}} & \numprint{75} & \textbf{\numprint{208}} & \numprint{211} & \textbf{\numprint{454}} & \numprint{465} & \textbf{\numprint{818}} & \numprint{849} & \textbf{\numprint{1361}} & \numprint{1391} & \textbf{\numprint{2143}} & \numprint{2211} & 
wing &       \textbf{\numprint{784}} & \numprint{787} & \textbf{\numprint{1616}} & \numprint{1666} & \textbf{\numprint{2509}} & \numprint{2589} & \textbf{\numprint{3889}} & \numprint{4131} & \textbf{\numprint{5747}} & \numprint{5902} & \textbf{\numprint{7842}} & \numprint{8132} & 
brack2 &       \textbf{\numprint{708}} & \numprint{708} & \textbf{\numprint{3013}} & \numprint{3027} & \textbf{\numprint{7110}} & \numprint{7144} & \textbf{\numprint{11745}} & \numprint{11969} & \textbf{\numprint{17751}} & \numprint{17798} & \numprint{26766} & \textbf{\numprint{26557}} & 
finan512 &       \textbf{\numprint{162}} & \numprint{162} & \textbf{\numprint{324}} & \numprint{324} & \textbf{\numprint{648}} & \numprint{648} & \textbf{\numprint{1296}} & \numprint{1296} & \textbf{\numprint{2592}} & \numprint{2592} & \numprint{10752} & \textbf{\numprint{10560}} & 
fe_tooth &       \textbf{\numprint{3815}} & \numprint{3819} & \textbf{\numprint{6870}} & \numprint{6938} & \textbf{\numprint{11492}} & \numprint{11650} & \textbf{\numprint{17592}} & \numprint{18115} & \textbf{\numprint{25695}} & \numprint{25977} & \textbf{\numprint{35722}} & \numprint{35980} & 
fe_rotor &       \textbf{\numprint{2031}} & \numprint{2045} & \numprint{7538} & \textbf{\numprint{7405}} & \numprint{13032} & \textbf{\numprint{12959}} & \numprint{20888} & \textbf{\numprint{20773}} & \textbf{\numprint{32678}} & \numprint{32783} & \numprint{47980} & \textbf{\numprint{47461}} & 
598a &       \textbf{\numprint{2388}} & \numprint{2388} & \textbf{\numprint{7956}} & \numprint{7992} & \textbf{\numprint{16050}} & \numprint{16179} & \textbf{\numprint{25892}} & \numprint{26196} & \textbf{\numprint{40003}} & \numprint{40513} & \textbf{\numprint{57795}} & \numprint{59098} & 
fe_ocean &       \textbf{\numprint{387}} & \numprint{387} & \textbf{\numprint{1831}} & \numprint{1856} & \textbf{\numprint{4140}} & \numprint{4251} & \textbf{\numprint{8035}} & \numprint{8276} & \textbf{\numprint{13224}} & \numprint{13660} & \textbf{\numprint{20828}} & \numprint{21548} & 
144 &       \textbf{\numprint{6478}} & \numprint{6479} & \numprint{15635} & \textbf{\numprint{15196}} & \textbf{\numprint{25281}} & \numprint{25455} & \textbf{\numprint{38221}} & \numprint{38940} & \textbf{\numprint{56897}} & \numprint{58126} & \textbf{\numprint{80451}} & \numprint{81145} & 
wave &       \textbf{\numprint{8665}} & \numprint{8682} & \textbf{\numprint{16881}} & \numprint{16891} & \textbf{\numprint{29124}} & \numprint{29207} & \textbf{\numprint{43027}} & \numprint{43697} & \textbf{\numprint{62567}} & \numprint{64198} & \textbf{\numprint{86127}} & \numprint{88863} & 
m14b &       \textbf{\numprint{3826}} & \numprint{3826} & \textbf{\numprint{12981}} & \numprint{13034} & \textbf{\numprint{25854}} & \numprint{25921} & \textbf{\numprint{42358}} & \numprint{42513} & \textbf{\numprint{67454}} & \numprint{67770} & \textbf{\numprint{99661}} & \numprint{101551} & 
auto &       \textbf{\numprint{9958}} & \numprint{10004} & \textbf{\numprint{26669}} & \numprint{26941} & \numprint{45892} & \textbf{\numprint{45731}} & \numprint{77743} & \textbf{\numprint{77618}} & \textbf{\numprint{121645}} & \numprint{123296} & \textbf{\numprint{174527}} & \numprint{175975} & 


==> tables/eps_3_ws_scratch.tex <==
3elt &       \textbf{\numprint{87}} & \numprint{87} & \textbf{\numprint{198}} & \numprint{198} & \textbf{\numprint{335}} & \numprint{336} & \textbf{\numprint{563}} & \numprint{565} & \numprint{962} & \textbf{\numprint{958}} & \numprint{1558} & \textbf{\numprint{1542}} & 
add20 &       \numprint{702} & \textbf{\numprint{576}} & \numprint{1186} & \textbf{\numprint{1158}} & \numprint{1724} & \textbf{\numprint{1690}} & \numprint{2104} & \textbf{\numprint{2095}} & \textbf{\numprint{2490}} & \numprint{2493} & \textbf{\numprint{3035}} & \numprint{3152} & 
data &       \textbf{\numprint{185}} & \numprint{185} & \textbf{\numprint{369}} & \numprint{378} & \textbf{\numprint{640}} & \numprint{650} & \textbf{\numprint{1127}} & \numprint{1133} & \numprint{1846} & \textbf{\numprint{1802}} & \numprint{2922} & \textbf{\numprint{2809}} & 
uk &       \textbf{\numprint{18}} & \numprint{18} & \textbf{\numprint{39}} & \numprint{40} & \textbf{\numprint{78}} & \numprint{81} & \textbf{\numprint{141}} & \numprint{148} & \textbf{\numprint{245}} & \numprint{251} & \numprint{418} & \textbf{\numprint{414}} & 
add32 &       \textbf{\numprint{10}} & \numprint{10} & \textbf{\numprint{30}} & \numprint{33} & \textbf{\numprint{66}} & \numprint{66} & \textbf{\numprint{117}} & \numprint{117} & \textbf{\numprint{212}} & \numprint{212} & \numprint{496} & \textbf{\numprint{493}} & 
bcsstk33 &       \textbf{\numprint{10064}} & \numprint{10064} & \textbf{\numprint{20865}} & \numprint{21035} & \textbf{\numprint{34078}} & \numprint{34078} & \numprint{54847} & \textbf{\numprint{54510}} & \numprint{78129} & \textbf{\numprint{77672}} & \numprint{108668} & \textbf{\numprint{107012}} & 
whitaker3 &       \textbf{\numprint{126}} & \numprint{126} & \textbf{\numprint{378}} & \numprint{378} & \textbf{\numprint{652}} & \numprint{655} & \textbf{\numprint{1090}} & \numprint{1092} & \textbf{\numprint{1680}} & \numprint{1686} & \numprint{2539} & \textbf{\numprint{2535}} & 
crack &       \textbf{\numprint{182}} & \numprint{182} & \textbf{\numprint{360}} & \numprint{360} & \textbf{\numprint{673}} & \numprint{676} & \numprint{1086} & \textbf{\numprint{1082}} & \numprint{1692} & \textbf{\numprint{1679}} & \numprint{2561} & \textbf{\numprint{2553}} & 
wing_nodal &       \textbf{\numprint{1678}} & \numprint{1680} & \textbf{\numprint{3545}} & \numprint{3561} & \textbf{\numprint{5374}} & \numprint{5401} & \textbf{\numprint{8315}} & \numprint{8316} & \numprint{11963} & \textbf{\numprint{11938}} & \numprint{16097} & \textbf{\numprint{15971}} & 
fe_4elt2 &       \textbf{\numprint{130}} & \numprint{130} & \textbf{\numprint{342}} & \numprint{343} & \textbf{\numprint{597}} & \numprint{598} & \textbf{\numprint{996}} & \numprint{1007} & \textbf{\numprint{1621}} & \numprint{1633} & \textbf{\numprint{2513}} & \numprint{2527} & 
vibrobox &       \numprint{11538} & \textbf{\numprint{10310}} & \numprint{18975} & \textbf{\numprint{18778}} & \numprint{24268} & \textbf{\numprint{24171}} & \numprint{33721} & \textbf{\numprint{31516}} & \numprint{42159} & \textbf{\numprint{39592}} & \numprint{49270} & \textbf{\numprint{49123}} & 
bcsstk29 &       \textbf{\numprint{2818}} & \numprint{2818} & \numprint{7993} & \textbf{\numprint{7983}} & \numprint{13867} & \textbf{\numprint{13817}} & \numprint{22494} & \textbf{\numprint{21410}} & \numprint{34892} & \textbf{\numprint{34407}} & \numprint{56682} & \textbf{\numprint{55366}} & 
4elt &       \textbf{\numprint{137}} & \numprint{137} & \textbf{\numprint{319}} & \numprint{319} & \textbf{\numprint{523}} & \numprint{523} & \numprint{918} & \textbf{\numprint{914}} & \numprint{1539} & \textbf{\numprint{1537}} & \textbf{\numprint{2570}} & \numprint{2581} & 
fe_sphere &       \textbf{\numprint{384}} & \numprint{384} & \textbf{\numprint{764}} & \numprint{764} & \textbf{\numprint{1152}} & \numprint{1152} & \textbf{\numprint{1705}} & \numprint{1706} & \numprint{2483} & \textbf{\numprint{2477}} & \numprint{3568} & \textbf{\numprint{3547}} & 
cti &       \textbf{\numprint{318}} & \numprint{318} & \textbf{\numprint{916}} & \numprint{917} & \textbf{\numprint{1714}} & \numprint{1716} & \textbf{\numprint{2773}} & \numprint{2778} & \textbf{\numprint{4029}} & \numprint{4132} & \textbf{\numprint{5683}} & \numprint{5763} & 
memplus &       \numprint{5466} & \textbf{\numprint{5355}} & \numprint{9593} & \textbf{\numprint{9418}} & \numprint{12085} & \textbf{\numprint{11628}} & \numprint{13384} & \textbf{\numprint{13130}} & \numprint{15124} & \textbf{\numprint{14264}} & \numprint{17183} & \textbf{\numprint{16724}} & 
cs4 &       \textbf{\numprint{360}} & \numprint{361} & \textbf{\numprint{928}} & \numprint{936} & \textbf{\numprint{1439}} & \numprint{1467} & \textbf{\numprint{2090}} & \numprint{2126} & \textbf{\numprint{2935}} & \numprint{3014} & \textbf{\numprint{4080}} & \numprint{4107} & 
bcsstk31 &       \textbf{\numprint{2676}} & \numprint{2676} & \textbf{\numprint{7150}} & \numprint{7181} & \textbf{\numprint{13020}} & \numprint{13246} & \numprint{23536} & \textbf{\numprint{23504}} & \numprint{38048} & \textbf{\numprint{37459}} & \numprint{58738} & \textbf{\numprint{58667}} & 
fe_pwt &       \textbf{\numprint{340}} & \numprint{340} & \textbf{\numprint{700}} & \numprint{704} & \textbf{\numprint{1411}} & \numprint{1416} & \textbf{\numprint{2776}} & \numprint{2784} & \textbf{\numprint{5496}} & \numprint{5606} & \textbf{\numprint{8228}} & \numprint{8346} & 
bcsstk32 &       \textbf{\numprint{4667}} & \numprint{4667} & \textbf{\numprint{8742}} & \numprint{8778} & \numprint{20223} & \textbf{\numprint{20035}} & \textbf{\numprint{35572}} & \numprint{35788} & \numprint{60766} & \textbf{\numprint{59824}} & \textbf{\numprint{92094}} & \numprint{92690} & 
fe_body &       \textbf{\numprint{262}} & \numprint{262} & \textbf{\numprint{598}} & \numprint{598} & \textbf{\numprint{1016}} & \numprint{1033} & \textbf{\numprint{1734}} & \numprint{1767} & \textbf{\numprint{2810}} & \numprint{2906} & \textbf{\numprint{4799}} & \numprint{4982} & 
t60k &       \textbf{\numprint{71}} & \numprint{71} & \textbf{\numprint{203}} & \numprint{207} & \textbf{\numprint{449}} & \numprint{454} & \textbf{\numprint{805}} & \numprint{822} & \textbf{\numprint{1343}} & \numprint{1391} & \textbf{\numprint{2115}} & \numprint{2198} & 
wing &       \textbf{\numprint{773}} & \numprint{774} & \textbf{\numprint{1605}} & \numprint{1636} & \textbf{\numprint{2471}} & \numprint{2551} & \textbf{\numprint{3862}} & \numprint{4015} & \textbf{\numprint{5645}} & \numprint{5832} & \textbf{\numprint{7727}} & \numprint{8043} & 
brack2 &       \textbf{\numprint{684}} & \numprint{684} & \textbf{\numprint{2834}} & \numprint{2839} & \textbf{\numprint{6871}} & \numprint{6980} & \textbf{\numprint{11462}} & \numprint{11622} & \textbf{\numprint{17211}} & \numprint{17491} & \textbf{\numprint{26026}} & \numprint{26366} & 
finan512 &       \textbf{\numprint{162}} & \numprint{162} & \textbf{\numprint{324}} & \numprint{324} & \textbf{\numprint{648}} & \numprint{648} & \textbf{\numprint{1296}} & \numprint{1296} & \textbf{\numprint{2592}} & \numprint{2592} & \numprint{10629} & \textbf{\numprint{10560}} & 
fe_tooth &       \textbf{\numprint{3788}} & \numprint{3792} & \textbf{\numprint{6796}} & \numprint{6862} & \textbf{\numprint{11313}} & \numprint{11422} & \textbf{\numprint{17318}} & \numprint{17655} & \textbf{\numprint{25208}} & \numprint{25624} & \textbf{\numprint{35044}} & \numprint{35830} & 
fe_rotor &       \textbf{\numprint{1959}} & \numprint{1960} & \textbf{\numprint{7128}} & \numprint{7182} & \textbf{\numprint{12479}} & \numprint{12546} & \numprint{20397} & \textbf{\numprint{20356}} & \textbf{\numprint{31345}} & \numprint{31763} & \textbf{\numprint{46783}} & \numprint{47049} & 
598a &       \textbf{\numprint{2367}} & \numprint{2367} & \textbf{\numprint{7842}} & \numprint{7873} & \textbf{\numprint{15740}} & \numprint{15820} & \textbf{\numprint{25704}} & \numprint{25927} & \textbf{\numprint{38803}} & \numprint{39525} & \textbf{\numprint{57070}} & \numprint{58101} & 
fe_ocean &       \textbf{\numprint{311}} & \numprint{311} & \textbf{\numprint{1696}} & \numprint{1698} & \textbf{\numprint{3921}} & \numprint{3974} & \textbf{\numprint{7648}} & \numprint{7838} & \textbf{\numprint{12550}} & \numprint{12746} & \textbf{\numprint{20049}} & \numprint{21033} & 
144 &       \textbf{\numprint{6438}} & \numprint{6438} & \numprint{15128} & \textbf{\numprint{15122}} & \textbf{\numprint{25119}} & \numprint{25301} & \textbf{\numprint{37782}} & \numprint{37899} & \textbf{\numprint{56399}} & \numprint{56463} & \textbf{\numprint{78626}} & \numprint{80621} & 
wave &       \textbf{\numprint{8594}} & \numprint{8616} & \textbf{\numprint{16668}} & \numprint{16822} & \textbf{\numprint{28513}} & \numprint{28664} & \textbf{\numprint{42308}} & \numprint{42620} & \textbf{\numprint{61756}} & \numprint{62281} & \textbf{\numprint{85254}} & \numprint{86663} & 
m14b &       \textbf{\numprint{3823}} & \numprint{3823} & \textbf{\numprint{12948}} & \numprint{12977} & \textbf{\numprint{25522}} & \numprint{25550} & \textbf{\numprint{42015}} & \numprint{42061} & \numprint{66401} & \textbf{\numprint{65879}} & \textbf{\numprint{96881}} & \numprint{100064} & 
auto &       \textbf{\numprint{9683}} & \numprint{9716} & \textbf{\numprint{25836}} & \numprint{25979} & \textbf{\numprint{44841}} & \numprint{45109} & \textbf{\numprint{75792}} & \numprint{76016} & \numprint{121581} & \textbf{\numprint{120534}} & \textbf{\numprint{0}} & \numprint{172357} & 


==> tables/eps_5_ws_scratch.tex <==
3elt &       \textbf{\numprint{87}} & \numprint{87} & \textbf{\numprint{197}} & \numprint{197} & \textbf{\numprint{330}} & \numprint{330} & \textbf{\numprint{558}} & \numprint{560} & \numprint{952} & \textbf{\numprint{950}} & \textbf{\numprint{1528}} & \numprint{1539} & 
add20 &       \numprint{691} & \textbf{\numprint{550}} & \numprint{1171} & \textbf{\numprint{1157}} & \numprint{1703} & \textbf{\numprint{1675}} & \numprint{2112} & \textbf{\numprint{2081}} & \textbf{\numprint{2440}} & \numprint{2463} & \numprint{2996} & \textbf{\numprint{1.0263}} & 
data &       \numprint{182} & \textbf{\numprint{181}} & \textbf{\numprint{363}} & \numprint{368} & \numprint{629} & \textbf{\numprint{628}} & \numprint{1092} & \textbf{\numprint{1086}} & \numprint{1813} & \textbf{\numprint{1777}} & \numprint{2852} & \textbf{\numprint{2798}} & 
uk &       \textbf{\numprint{18}} & \numprint{18} & \textbf{\numprint{39}} & \numprint{39} & \textbf{\numprint{76}} & \numprint{78} & \textbf{\numprint{139}} & \numprint{139} & \textbf{\numprint{242}} & \numprint{246} & \textbf{\numprint{404}} & \numprint{410} & 
add32 &       \textbf{\numprint{10}} & \numprint{10} & \numprint{30} & \textbf{\numprint{1.0008}} & \textbf{\numprint{63}} & \numprint{63} & \textbf{\numprint{117}} & \numprint{117} & \textbf{\numprint{212}} & \numprint{212} & \textbf{\numprint{486}} & \numprint{491} & 
bcsstk33 &       \textbf{\numprint{9914}} & \numprint{9914} & \numprint{20216} & \textbf{\numprint{20198}} & \textbf{\numprint{33922}} & \numprint{33938} & \numprint{54692} & \textbf{\numprint{54323}} & \numprint{77564} & \textbf{\numprint{77163}} & \numprint{107832} & \textbf{\numprint{106886}} & 
whitaker3 &       \textbf{\numprint{126}} & \numprint{126} & \textbf{\numprint{378}} & \numprint{378} & \textbf{\numprint{647}} & \numprint{650} & \numprint{1087} & \textbf{\numprint{1084}} & \textbf{\numprint{1673}} & \numprint{1686} & \textbf{\numprint{2512}} & \numprint{2535} & 
crack &       \textbf{\numprint{182}} & \numprint{182} & \textbf{\numprint{360}} & \numprint{360} & \textbf{\numprint{667}} & \numprint{667} & \textbf{\numprint{1077}} & \numprint{1080} & \numprint{1682} & \textbf{\numprint{1679}} & \textbf{\numprint{2526}} & \numprint{2548} & 
wing_nodal &       \numprint{1669} & \textbf{\numprint{1668}} & \textbf{\numprint{3524}} & \numprint{3536} & \textbf{\numprint{5346}} & \numprint{5350} & \textbf{\numprint{8266}} & \numprint{8316} & \textbf{\numprint{11855}} & \numprint{11879} & \numprint{16111} & \textbf{\numprint{15873}} & 
fe_4elt2 &       \textbf{\numprint{130}} & \numprint{130} & \textbf{\numprint{335}} & \numprint{335} & \textbf{\numprint{581}} & \numprint{583} & \textbf{\numprint{986}} & \numprint{991} & \textbf{\numprint{1600}} & \numprint{1633} & \textbf{\numprint{2493}} & \numprint{2516} & 
vibrobox &       \numprint{11486} & \textbf{\numprint{10310}} & \numprint{18856} & \textbf{\numprint{18778}} & \numprint{23948} & \textbf{\numprint{23930}} & \numprint{33113} & \textbf{\numprint{31235}} & \numprint{41812} & \textbf{\numprint{39592}} & \numprint{48841} & \textbf{\numprint{48200}} & 
bcsstk29 &       \textbf{\numprint{2818}} & \numprint{2818} & \numprint{7942} & \textbf{\numprint{7936}} & \textbf{\numprint{13575}} & \numprint{13614} & \numprint{21971} & \textbf{\numprint{20924}} & \numprint{34452} & \textbf{\numprint{33818}} & \numprint{55873} & \textbf{\numprint{54935}} & 
4elt &       \textbf{\numprint{137}} & \numprint{137} & \textbf{\numprint{315}} & \numprint{315} & \textbf{\numprint{516}} & \numprint{516} & \textbf{\numprint{901}} & \numprint{902} & \textbf{\numprint{1520}} & \numprint{1532} & \textbf{\numprint{2554}} & \numprint{2565} & 
fe_sphere &       \textbf{\numprint{384}} & \numprint{384} & \textbf{\numprint{762}} & \numprint{764} & \textbf{\numprint{1152}} & \numprint{1152} & \textbf{\numprint{1688}} & \numprint{1692} & \textbf{\numprint{2433}} & \numprint{2477} & \textbf{\numprint{3535}} & \numprint{3547} & 
cti &       \textbf{\numprint{318}} & \numprint{318} & \textbf{\numprint{889}} & \numprint{890} & \textbf{\numprint{1684}} & \numprint{1708} & \numprint{2735} & \textbf{\numprint{2725}} & \textbf{\numprint{3957}} & \numprint{4037} & \textbf{\numprint{5609}} & \numprint{5684} & 
memplus &       \numprint{5362} & \textbf{\numprint{5267}} & \numprint{9690} & \textbf{\numprint{9299}} & \numprint{12078} & \textbf{\numprint{11555}} & \numprint{13349} & \textbf{\numprint{13078}} & \numprint{14992} & \textbf{\numprint{14170}} & \numprint{16758} & \textbf{\numprint{16454}} & 
cs4 &       \textbf{\numprint{353}} & \numprint{356} & \textbf{\numprint{922}} & \numprint{936} & \textbf{\numprint{1435}} & \numprint{1467} & \textbf{\numprint{2083}} & \numprint{2126} & \textbf{\numprint{2923}} & \numprint{2958} & \numprint{4055} & \textbf{\numprint{4052}} & 
bcsstk31 &       \textbf{\numprint{2670}} & \numprint{2676} & \textbf{\numprint{7088}} & \numprint{7099} & \textbf{\numprint{12865}} & \numprint{12941} & \textbf{\numprint{23202}} & \numprint{23254} & \textbf{\numprint{37282}} & \numprint{37459} & \numprint{57748} & \textbf{\numprint{57534}} & 
fe_pwt &       \textbf{\numprint{340}} & \numprint{340} & \textbf{\numprint{700}} & \numprint{700} & \textbf{\numprint{1405}} & \numprint{1405} & \textbf{\numprint{2748}} & \numprint{2772} & \textbf{\numprint{5431}} & \numprint{5545} & \textbf{\numprint{8136}} & \numprint{8310} & 
bcsstk32 &       \textbf{\numprint{4622}} & \numprint{4622} & \textbf{\numprint{8441}} & \numprint{8454} & \textbf{\numprint{19601}} & \numprint{19678} & \textbf{\numprint{35014}} & \numprint{35208} & \textbf{\numprint{59456}} & \numprint{59824} & \numprint{91110} & \textbf{\numprint{91006}} & 
fe_body &       \textbf{\numprint{262}} & \numprint{262} & \textbf{\numprint{589}} & \numprint{596} & \textbf{\numprint{1014}} & \numprint{1017} & \textbf{\numprint{1701}} & \numprint{1723} & \textbf{\numprint{2787}} & \numprint{2807} & \textbf{\numprint{4642}} & \numprint{4834} & 
t60k &       \textbf{\numprint{65}} & \numprint{65} & \textbf{\numprint{195}} & \numprint{196} & \textbf{\numprint{445}} & \numprint{454} & \textbf{\numprint{801}} & \numprint{818} & \textbf{\numprint{1337}} & \numprint{1376} & \textbf{\numprint{2106}} & \numprint{2168} & 
wing &       \textbf{\numprint{770}} & \numprint{770} & \textbf{\numprint{1597}} & \numprint{1636} & \textbf{\numprint{2456}} & \numprint{2528} & \textbf{\numprint{3842}} & \numprint{3998} & \textbf{\numprint{5586}} & \numprint{5806} & \textbf{\numprint{7651}} & \numprint{7991} & 
brack2 &       \textbf{\numprint{660}} & \numprint{660} & \textbf{\numprint{2731}} & \numprint{2739} & \textbf{\numprint{6634}} & \numprint{6671} & \textbf{\numprint{11240}} & \numprint{11358} & \textbf{\numprint{17137}} & \numprint{17256} & \textbf{\numprint{25827}} & \numprint{26281} & 
finan512 &       \textbf{\numprint{162}} & \numprint{162} & \textbf{\numprint{324}} & \numprint{324} & \textbf{\numprint{648}} & \numprint{648} & \textbf{\numprint{1296}} & \numprint{1296} & \textbf{\numprint{2592}} & \numprint{2592} & \numprint{10604} & \textbf{\numprint{10560}} & 
fe_tooth &       \textbf{\numprint{3773}} & \numprint{3773} & \textbf{\numprint{6718}} & \numprint{6825} & \textbf{\numprint{11185}} & \numprint{11337} & \textbf{\numprint{17230}} & \numprint{17404} & \textbf{\numprint{24977}} & \numprint{25216} & \textbf{\numprint{34704}} & \numprint{35466} & 
fe_rotor &       \textbf{\numprint{1940}} & \numprint{1950} & \textbf{\numprint{6999}} & \numprint{7045} & \textbf{\numprint{12353}} & \numprint{12380} & \textbf{\numprint{19935}} & \numprint{20132} & \textbf{\numprint{31016}} & \numprint{31450} & \textbf{\numprint{46006}} & \numprint{46608} & 
598a &       \textbf{\numprint{2336}} & \numprint{2336} & \textbf{\numprint{7738}} & \numprint{7763} & \textbf{\numprint{15502}} & \numprint{15544} & \textbf{\numprint{25560}} & \numprint{25585} & \textbf{\numprint{38884}} & \numprint{39144} & \textbf{\numprint{56586}} & \numprint{57412} & 
fe_ocean &       \textbf{\numprint{311}} & \numprint{311} & \textbf{\numprint{1686}} & \numprint{1697} & \textbf{\numprint{3902}} & \numprint{3941} & \textbf{\numprint{7457}} & \numprint{7618} & \textbf{\numprint{12373}} & \numprint{12720} & \textbf{\numprint{19764}} & \numprint{20667} & 
144 &       \textbf{\numprint{6361}} & \numprint{6362} & \numprint{15321} & \textbf{\numprint{15122}} & \numprint{25078} & \textbf{\numprint{25025}} & \numprint{37505} & \textbf{\numprint{37433}} & \textbf{\numprint{56041}} & \numprint{56463} & \textbf{\numprint{78645}} & \numprint{79296} & 
wave &       \textbf{\numprint{8535}} & \numprint{8563} & \textbf{\numprint{16543}} & \numprint{16662} & \textbf{\numprint{28493}} & \numprint{28615} & \textbf{\numprint{42179}} & \numprint{42482} & \textbf{\numprint{61386}} & \numprint{61788} & \textbf{\numprint{84247}} & \numprint{85658} & 
m14b &       \textbf{\numprint{3802}} & \numprint{3802} & \textbf{\numprint{12945}} & \numprint{12976} & \numprint{25296} & \textbf{\numprint{25292}} & \numprint{41753} & \textbf{\numprint{41750}} & \numprint{65910} & \textbf{\numprint{65231}} & \textbf{\numprint{96580}} & \numprint{98005} & 
auto &       \textbf{\numprint{9450}} & \numprint{9450} & \textbf{\numprint{25310}} & \numprint{25399} & \textbf{\numprint{44360}} & \numprint{44520} & \textbf{\numprint{0}} & \numprint{75066} & \textbf{\numprint{0}} & \numprint{120001} & \textbf{\numprint{0}} & \numprint{171459} & 


==> tables/raw_tex_data_improve_5.tex <==
3elt &       \numprint{87} & \textbf{\numprint{87}} & \numprint{197} & \textbf{\numprint{197}} & \numprint{330} & \textbf{\numprint{330}} & \textbf{\numprint{558}} & \numprint{558} & \textbf{\numprint{942}} & \numprint{950} & \textbf{\numprint{1519}} & \numprint{1528} \\
add20 &       \numprint{550} & \textbf{\numprint{550}} & \textbf{\numprint{1149}} & \numprint{1157} & \numprint{1675} & \textbf{\numprint{1675}} & \numprint{2081} & \textbf{\numprint{2081}} & \numprint{2440} & \textbf{\numprint{2440}} & \numprint{3152} & \textbf{\numprint{3152}} \\
data &       \numprint{181} & \textbf{\numprint{181}} & \numprint{363} & \textbf{\numprint{363}} & \numprint{628} & \textbf{\numprint{628}} & \textbf{\numprint{1084}} & \numprint{1086} & \textbf{\numprint{1776}} & \numprint{1777} & \numprint{2798} & \textbf{\numprint{2798}} \\
uk &       \numprint{18} & \textbf{\numprint{18}} & \textbf{\numprint{39}} & \numprint{39} & \numprint{76} & \textbf{\numprint{76}} & \textbf{\numprint{139}} & \numprint{139} & \numprint{242} & \textbf{\numprint{242}} & \textbf{\numprint{400}} & \numprint{404} \\
add32 &       \numprint{10} & \textbf{\numprint{10}} & \numprint{33} & \textbf{\numprint{33}} & \numprint{63} & \textbf{\numprint{63}} & \numprint{117} & \textbf{\numprint{117}} & \numprint{212} & \textbf{\numprint{212}} & \numprint{486} & \textbf{\numprint{486}} \\
bcsstk33 &       \numprint{9914} & \textbf{\numprint{9914}} & \textbf{\numprint{20179}} & \numprint{20198} & \numprint{33922} & \textbf{\numprint{33922}} & \textbf{\numprint{54296}} & \numprint{54323} & \textbf{\numprint{77101}} & \numprint{77163} & \textbf{\numprint{106827}} & \numprint{106886} \\
whitaker3 &       \numprint{126} & \textbf{\numprint{126}} & \numprint{378} & \textbf{\numprint{378}} & \textbf{\numprint{644}} & \numprint{647} & \textbf{\numprint{1079}} & \numprint{1084} & \textbf{\numprint{1667}} & \numprint{1673} & \textbf{\numprint{2498}} & \numprint{2512} \\
crack &       \numprint{182} & \textbf{\numprint{182}} & \numprint{360} & \textbf{\numprint{360}} & \textbf{\numprint{667}} & \numprint{667} & \textbf{\numprint{1076}} & \numprint{1077} & \textbf{\numprint{1655}} & \numprint{1679} & \textbf{\numprint{2516}} & \numprint{2526} \\
wing\_nodal &       \numprint{1668} & \textbf{\numprint{1668}} & \textbf{\numprint{3522}} & \numprint{3524} & \textbf{\numprint{5345}} & \numprint{5346} & \textbf{\numprint{8264}} & \numprint{8266} & \textbf{\numprint{11844}} & \numprint{11855} & \textbf{\numprint{15813}} & \numprint{15873} \\
fe\_4elt2 &       \numprint{130} & \textbf{\numprint{130}} & \textbf{\numprint{335}} & \numprint{335} & \textbf{\numprint{580}} & \numprint{581} & \textbf{\numprint{984}} & \numprint{986} & \textbf{\numprint{1592}} & \numprint{1600} & \textbf{\numprint{2482}} & \numprint{2493} \\
vibrobox &       \numprint{10310} & \textbf{\numprint{10310}} & \textbf{\numprint{18696}} & \numprint{18778} & \numprint{23930} & \textbf{\numprint{23930}} & \textbf{\numprint{31234}} & \numprint{31235} & \textbf{\numprint{39183}} & \numprint{39592} & \textbf{\numprint{47361}} & \numprint{48200} \\
bcsstk29 &       \numprint{2818} & \textbf{\numprint{2818}} & \numprint{7936} & \textbf{\numprint{7936}} & \numprint{13575} & \textbf{\numprint{13575}} & \numprint{20924} & \textbf{\numprint{20924}} & \textbf{\numprint{33817}} & \numprint{33818} & \textbf{\numprint{54895}} & \numprint{54935} \\
4elt &       \numprint{137} & \textbf{\numprint{137}} & \numprint{315} & \textbf{\numprint{315}} & \textbf{\numprint{515}} & \numprint{516} & \textbf{\numprint{895}} & \numprint{901} & \textbf{\numprint{1516}} & \numprint{1520} & \textbf{\numprint{2546}} & \numprint{2554} \\
fe\_sphere &       \numprint{384} & \textbf{\numprint{384}} & \textbf{\numprint{762}} & \numprint{762} & \numprint{1152} & \textbf{\numprint{1152}} & \textbf{\numprint{1683}} & \numprint{1688} & \textbf{\numprint{2465}} & \numprint{2477} & \textbf{\numprint{3522}} & \numprint{3547} \\
cti &       \numprint{318} & \textbf{\numprint{318}} & \numprint{889} & \textbf{\numprint{889}} & \textbf{\numprint{1684}} & \numprint{1684} & \textbf{\numprint{2721}} & \numprint{2725} & \textbf{\numprint{3920}} & \numprint{3957} & \textbf{\numprint{5594}} & \numprint{5609} \\
memplus &       \numprint{5267} & \textbf{\numprint{5267}} & \textbf{\numprint{9297}} & \numprint{9299} & \textbf{\numprint{11543}} & \numprint{11555} & \textbf{\numprint{13061}} & \numprint{13078} & \textbf{\numprint{14152}} & \numprint{14170} & \textbf{\numprint{16044}} & \numprint{16454} \\
cs4 &       \numprint{353} & \textbf{\numprint{353}} & \textbf{\numprint{912}} & \numprint{922} & \textbf{\numprint{1431}} & \numprint{1435} & \textbf{\numprint{2079}} & \numprint{2083} & \textbf{\numprint{2919}} & \numprint{2923} & \textbf{\numprint{4012}} & \numprint{4052} \\
bcsstk31 &       \textbf{\numprint{2670}} & \numprint{2670} & \textbf{\numprint{7088}} & \numprint{7088} & \textbf{\numprint{12865}} & \numprint{12865} & \textbf{\numprint{23104}} & \numprint{23202} & \textbf{\numprint{37261}} & \numprint{37282} & \textbf{\numprint{56674}} & \numprint{57534} \\
fe\_pwt &       \numprint{340} & \textbf{\numprint{340}} & \numprint{700} & \textbf{\numprint{700}} & \textbf{\numprint{1405}} & \numprint{1405} & \textbf{\numprint{2745}} & \numprint{2748} & \textbf{\numprint{5423}} & \numprint{5431} & \textbf{\numprint{8119}} & \numprint{8136} \\
bcsstk32 &       \numprint{4622} & \textbf{\numprint{4622}} & \numprint{8441} & \textbf{\numprint{8441}} & \textbf{\numprint{19601}} & \numprint{19601} & \numprint{35014} & \textbf{\numprint{35014}} & \textbf{\numprint{59248}} & \numprint{59456} & \textbf{\numprint{89897}} & \numprint{91006} \\
fe\_body &       \numprint{262} & \textbf{\numprint{262}} & \textbf{\numprint{588}} & \numprint{589} & \textbf{\numprint{1014}} & \numprint{1014} & \textbf{\numprint{1697}} & \numprint{1701} & \numprint{2787} & \textbf{\numprint{2787}} & \numprint{4642} & \textbf{\numprint{4642}} \\
t60k &       \numprint{65} & \textbf{\numprint{65}} & \textbf{\numprint{195}} & \numprint{195} & \textbf{\numprint{445}} & \numprint{445} & \textbf{\numprint{796}} & \numprint{801} & \textbf{\numprint{1329}} & \numprint{1337} & \textbf{\numprint{2089}} & \numprint{2106} \\
wing &       \textbf{\numprint{770}} & \numprint{770} & \textbf{\numprint{1593}} & \numprint{1597} & \textbf{\numprint{2452}} & \numprint{2456} & \textbf{\numprint{3832}} & \numprint{3842} & \textbf{\numprint{5564}} & \numprint{5586} & \textbf{\numprint{7611}} & \numprint{7651} \\
brack2 &       \numprint{660} & \textbf{\numprint{660}} & \numprint{2731} & \textbf{\numprint{2731}} & \textbf{\numprint{6611}} & \numprint{6634} & \textbf{\numprint{11232}} & \numprint{11240} & \textbf{\numprint{17112}} & \numprint{17137} & \textbf{\numprint{25805}} & \numprint{25827} \\
finan512 &       \numprint{162} & \textbf{\numprint{162}} & \numprint{324} & \textbf{\numprint{324}} & \numprint{648} & \textbf{\numprint{648}} & \numprint{1296} & \textbf{\numprint{1296}} & \numprint{2592} & \textbf{\numprint{2592}} & \numprint{10560} & \textbf{\numprint{10560}} \\
fe\_tooth &       \numprint{3773} & \textbf{\numprint{3773}} & \textbf{\numprint{6714}} & \numprint{6718} & \numprint{11185} & \textbf{\numprint{11185}} & \textbf{\numprint{17215}} & \numprint{17230} & \textbf{\numprint{24957}} & \numprint{24977} & \textbf{\numprint{34698}} & \numprint{34704} \\
fe\_rotor &       \numprint{1940} & \textbf{\numprint{1940}} & \textbf{\numprint{6940}} & \numprint{6999} & \textbf{\numprint{12347}} & \numprint{12353} & \textbf{\numprint{19932}} & \numprint{19935} & \textbf{\numprint{30974}} & \numprint{31016} & \textbf{\numprint{45931}} & \numprint{46006} \\
598a &       \numprint{2336} & \textbf{\numprint{2336}} & \textbf{\numprint{7735}} & \numprint{7738} & \textbf{\numprint{15483}} & \numprint{15502} & \textbf{\numprint{25533}} & \numprint{25560} & \textbf{\numprint{38550}} & \numprint{38803} & \textbf{\numprint{56551}} & \numprint{56586} \\
fe\_ocean &       \numprint{311} & \textbf{\numprint{311}} & \numprint{1686} & \textbf{\numprint{1686}} & \textbf{\numprint{3902}} & \numprint{3902} & \textbf{\numprint{7412}} & \numprint{7457} & \textbf{\numprint{12362}} & \numprint{12373} & \textbf{\numprint{19727}} & \numprint{19764} \\
144 &       \textbf{\numprint{6359}} & \numprint{6361} & \textbf{\numprint{14982}} & \numprint{15122} & \textbf{\numprint{24767}} & \numprint{25025} & \textbf{\numprint{37122}} & \numprint{37433} & \textbf{\numprint{55984}} & \numprint{56041} & \textbf{\numprint{78069}} & \numprint{78626} \\
wave &       \textbf{\numprint{8533}} & \numprint{8535} & \textbf{\numprint{16533}} & \numprint{16543} & \textbf{\numprint{28492}} & \numprint{28493} & \textbf{\numprint{42134}} & \numprint{42179} & \textbf{\numprint{61280}} & \numprint{61386} & \textbf{\numprint{84236}} & \numprint{84247} \\
m14b &       \numprint{3802} & \textbf{\numprint{3802}} & \textbf{\numprint{12945}} & \numprint{12945} & \textbf{\numprint{25143}} & \numprint{25151} & \textbf{\numprint{41536}} & \numprint{41538} & \textbf{\numprint{65077}} & \numprint{65087} & \textbf{\numprint{96559}} & \numprint{96580} \\
auto &       \numprint{9450} & \textbf{\numprint{9450}} & \textbf{\numprint{25301}} & \numprint{25310} & \textbf{\numprint{44346}} & \numprint{44360} & \textbf{\numprint{74561}} & \numprint{75066} & \textbf{\numprint{119111}} & \numprint{119125} & \textbf{\numprint{171329}} & \numprint{171355} \\


==> tables/walshaw-improve-KaFFPa-eps-1.tex <==

\begin{landscape}
\begin{table}[H]
\begin{center}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|}\hline

 Graph  & \multicolumn{2}{|c|}{2} & \multicolumn{2}{|c|}{4} & \multicolumn{2}{|c|}{8} & \multicolumn{2}{|c|}{16} & \multicolumn{2}{|c|}{32} & \multicolumn{2}{|c|}{64}\\

\hline 
 3elt      & 89             & \textbf{89}    & 199            & \textbf{199}   & \textbf{341}   & 342            & 569            & \textbf{569}   & 969             & \textbf{969}  & \textbf{1553}   & 1564  \\
 add20     & 594            & \textbf{594}   & 1177           & \textbf{1177}  & \textbf{1703}  & 1704           & \textbf{2118}  & 2121           & \textbf{2623}   & 2687          & \textbf{3090}   & 3236  \\
 data      & 188            & \textbf{188}   & \textbf{381}   & 383            & 660            & \textbf{660}   & \textbf{1161}  & 1162           & \textbf{1863}   & 1865          & 2885            & \textbf{2885}  \\
 uk        & 19             & \textbf{19}    & 41             & \textbf{41}    & 84             & \textbf{84}    & 152            & \textbf{152}   & 258             & \textbf{258}  & \textbf{422}    & 438  \\
 add32     & 10             & \textbf{10}    & 33             & \textbf{33}    & 66             & \textbf{66}    & 117            & \textbf{117}   & 212             & \textbf{212}  & 493             & \textbf{493}  \\
 bcsstk33  & \textbf{10096} & 10097          & 21508          & \textbf{21508} & 34178          & \textbf{34178} & 54860          & \textbf{54860} & \textbf{78069}  & 78132         & \textbf{108490} & 108505  \\
 whitaker3 & 126            & \textbf{126}   & 380            & \textbf{380}   & \textbf{655}   & 656            & \textbf{1092}  & 1093           & \textbf{1707}   & 1717          & \textbf{2557}   & 2567  \\
 crack     & 183            & \textbf{183}   & 362            & \textbf{362}   & 678            & \textbf{678}   & \textbf{1091}  & 1092           & \textbf{1701}   & 1707          & \textbf{2555}   & 2566  \\
 wingnodal & 1696           & \textbf{1696}  & \textbf{3570}  & 3572           & \textbf{5438}  & 5443           & \textbf{8366}  & 8422           & \textbf{11979}  & 11980         & \textbf{16128}  & 16134  \\
 fe4elt2   & 130            & \textbf{130}   & 349            & \textbf{349}   & 605            & \textbf{605}   & \textbf{1010}  & 1014           & \textbf{1643}   & 1657          & \textbf{2517}   & 2537  \\
 vibrobox  & 10310          & \textbf{10310} & \textbf{19196} & 19199          & \textbf{24549} & 24553          & \textbf{32116} & 32167          & \textbf{40812}  & 41399         & \textbf{49136}  & 49521  \\
 bcsstk29  & 2818           & \textbf{2818}  & \textbf{8029}  & 8035           & \textbf{13950} & 13965          & 21768          & \textbf{21768} & \textbf{34875}  & 34886         & \textbf{57053}  & 57054  \\
 4elt      & 138            & \textbf{138}   & 321            & \textbf{321}   & 534            & \textbf{534}   & \textbf{935}   & 939            & \textbf{1547}   & 1559          & \textbf{2580}   & 2596  \\
 fesphere  & 386            & \textbf{386}   & 768            & \textbf{768}   & 1152           & \textbf{1152}  & \textbf{1714}  & 1730           & \textbf{2525}   & 2565          & \textbf{3576}   & 3663  \\
 cti       & 318            & \textbf{318}   & 944            & \textbf{944}   & 1802           & \textbf{1802}  & \textbf{2894}  & 2906           & 4223            & \textbf{4223} & \textbf{5872}   & 5875  \\
 memplus   & \textbf{5485}  & 5489           & \textbf{9544}  & 9559           & \textbf{11777} & 11785          & \textbf{13237} & 13241          & \textbf{14358}  & 14395         & \textbf{16626}  & 16857  \\
 cs4       & 367            & \textbf{367}   & \textbf{938}   & 940            & 1467           & \textbf{1467}  & 2195           & \textbf{2195}  & \textbf{3040}   & 3048          & \textbf{4145}   & 4154  \\
 bcsstk31  & 2701           & \textbf{2701}  & 7444           & \textbf{7444}  & \textbf{13306} & 13371          & \textbf{24225} & 24277          & \textbf{38014}  & 38086         & \textbf{60162}  & 60528  \\
 fepwt     & 340            & \textbf{340}   & 704            & \textbf{704}   & \textbf{1439}  & 1441           & \textbf{2803}  & 2806           & \textbf{5551}   & 5612          & \textbf{8426}   & 8454  \\
 bcsstk32  & 4667           & \textbf{4667}  & 9247           & \textbf{9247}  & \textbf{20701} & 20855          & \textbf{37186} & 37372          & \textbf{61114}  & 61144         & \textbf{94443}  & 95199  \\
 febody    & 262            & \textbf{262}   & \textbf{598}   & 599            & \textbf{1068}  & 1079           & \textbf{1818}  & 1858           & \textbf{3105}   & 3202          & \textbf{5126}   & 5282  \\
 t60k      & 75             & \textbf{75}    & 211            & \textbf{211}   & \textbf{463}   & 465            & 849            & \textbf{849}   & \textbf{1389}   & 1391          & \textbf{2192}   & 2211  \\
 wing      & 787            & \textbf{787}   & \textbf{1653}  & 1666           & \textbf{2521}  & 2589           & \textbf{4126}  & 4131           & \textbf{5879}   & 5902          & \textbf{8055}   & 8132  \\
 brack2    & 708            & \textbf{708}   & \textbf{3019}  & 3027           & \textbf{7103}  & 7144           & \textbf{11852} & 11969          & \textbf{17745}  & 17798         & \textbf{26456}  & 26557  \\
 finan512  & 162            & \textbf{162}   & 324            & \textbf{324}   & 648            & \textbf{648}   & 1296           & \textbf{1296}  & 2592            & \textbf{2592} & 10560           & \textbf{10560}  \\
 fetooth   & \textbf{3817}  & 3819           & \textbf{6917}  & 6938           & \textbf{11566} & 11650          & \textbf{17935} & 18115          & \textbf{25349}  & 25977         & \textbf{35581}  & 35980  \\
 ferotor   & \textbf{2033}  & 2045           & \textbf{7316}  & 7405           & \textbf{12869} & 12959          & \textbf{20707} & 20773          & \textbf{32429}  & 32783         & \textbf{47087}  & 47461  \\
 598a      & 2388           & \textbf{2388}  & \textbf{7978}  & 7992           & \textbf{16105} & 16179          & \textbf{26095} & 26196          & \textbf{40196}  & 40513         & \textbf{57411}  & 59098  \\
 feocean   & 387            & \textbf{387}   & \textbf{1852}  & 1856           & \textbf{4188}  & 4251           & \textbf{8141}  & 8276           & \textbf{13256}  & 13660         & \textbf{21054}  & 21548  \\
 144       & 6479           & \textbf{6479}  & \textbf{15179} & 15196          & \textbf{25420} & 25455          & \textbf{38691} & 38940          & \textbf{56510}  & 58126         & \textbf{80357}  & 81145  \\
 wave      & \textbf{8681}  & 8682           & \textbf{16829} & 16891          & \textbf{29095} & 29207          & \textbf{43396} & 43697          & \textbf{63650}  & 64198         & \textbf{86699}  & 88863  \\
 m14b      & 3826           & \textbf{3826}  & \textbf{13025} & 13034          & \textbf{25843} & 25921          & \textbf{42448} & 42513          & \textbf{66497}  & 67770         & \textbf{98703}  & 101551  \\
 auto      & \textbf{9980}  & 10004          & \textbf{26761} & 26941          & \textbf{45572} & 45731          & \textbf{77312} & 77618          & \textbf{122637} & 123296        & \textbf{172884} & 175975  \\
 \hline

\end{tabular}
 \end{center} \caption{Improveing existing partitions $\epsilon = 1$\%}
\end{table}

\end{landscape}


==> tables/walshaw-improve-KaFFPa-eps-3.tex <==

\begin{landscape}
\begin{table}[H]
\begin{center}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|}\hline

 Graph  & \multicolumn{2}{|c|}{2} & \multicolumn{2}{|c|}{4} & \multicolumn{2}{|c|}{8} & \multicolumn{2}{|c|}{16} & \multicolumn{2}{|c|}{32} & \multicolumn{2}{|c|}{64}\\

\hline 
 3elt & 	 87 & 	 \textbf{87} & 	 198 & 	 \textbf{198} & 	 336 & 	 \textbf{336} & 	 \textbf{564} & 	 565 & 	 \textbf{950} & 	 958 & 	 \textbf{1533} & 	 1542  \\ 
 add20 & 	 576 & 	 \textbf{576} & 	 1158 & 	 \textbf{1158} & 	 1690 & 	 \textbf{1690} & 	 \textbf{2087} & 	 2095 & 	 \textbf{2481} & 	 2493 & 	  \textbf{3104} & 	 3152  \\ 
 data & 	 185 & 	 \textbf{185} & 	 378 & 	 \textbf{378} & 	 650 & 	 \textbf{650} & 	 \textbf{1124} & 	 1133 & 	 1802 & 	 \textbf{1802} & 	 2809 & 	 \textbf{2809}  \\ 
 uk & 	 18 & 	 \textbf{18} & 	 40 & 	 \textbf{40} & 	 81 & 	 \textbf{81} & 	 \textbf{147} & 	 148 & 	 251 & 	 \textbf{251} & 	 \textbf{413} & 	 414  \\ 
 add32 & 	 10 & 	 \textbf{10} & 	 33 & 	 \textbf{33} & 	 66 & 	 \textbf{66} & 	 117 & 	 \textbf{117} & 	 212 & 	 \textbf{212} & 	 \textbf{490} & 	 493  \\ 
 bcsstk33 & 	 10064 & 	 \textbf{10064} & 	 21035 & 	 \textbf{21035} & 	 34078 & 	 \textbf{34078} & 	 \textbf{54490} & 	 54510 & 	 \textbf{77657} & 	 77672 & 	 \textbf{107011} & 	 107012  \\ 
 whitaker3 & 	 126 & 	 \textbf{126} & 	 378 & 	 \textbf{378} & 	 \textbf{654} & 	 655 & 	 \textbf{1087} & 	 1092 & 	 \textbf{1679} & 	 1686 & 	 \textbf{2503} & 	 2535  \\ 
 crack & 	 182 & 	 \textbf{182} & 	 360 & 	 \textbf{360} & 	 \textbf{675} & 	 676 & 	 \textbf{1079} & 	 1082 & 	 \textbf{1667} & 	 1679 & 	 \textbf{2535} & 	 2553  \\ 
 wingnodal & 	 1680 & 	 \textbf{1680} & 	 \textbf{3556} & 	 3561 & 	 \textbf{5387} & 	 5401 & 	 \textbf{8299} & 	 8316 & 	 \textbf{11931} & 	 11938 & 	 \textbf{15963} & 	 15971  \\ 
 fe4elt2 & 	 130 & 	 \textbf{130} & 	 343 & 	 \textbf{343} & 	 598 & 	 \textbf{598} & 	 \textbf{999} & 	 1007 & 	 \textbf{1617} & 	 1633 & 	 \textbf{2495} & 	 2527  \\ 
 vibrobox & 	 10310 & 	 \textbf{10310} & 	 18778 & 	 \textbf{18778} & 	 \textbf{24170} & 	 24171 & 	 \textbf{31515} & 	 31516 & 	 \textbf{39577} & 	 39592 & 	 \textbf{48791} & 	 49123  \\ 
 bcsstk29 & 	 2818 & 	 \textbf{2818} & 	 7983 & 	 \textbf{7983} & 	 13817 & 	 \textbf{13817} & 	 21410 & 	 \textbf{21410} & 	 \textbf{34402} & 	 34407 & 	 \textbf{55328} & 	 55366  \\ 
 4elt & 	 137 & 	 \textbf{137} & 	 319 & 	 \textbf{319} & 	 523 & 	 \textbf{523} & 	 \textbf{909} & 	 914 & 	 \textbf{1525} & 	 1537 & 	 \textbf{2557} & 	 2581  \\ 
 fesphere & 	 384 & 	 \textbf{384} & 	 764 & 	 \textbf{764} & 	 1152 & 	 \textbf{1152} & 	 \textbf{1705} & 	 1706 & 	 \textbf{2473} & 	 2477 & 	 \textbf{3526} & 	 3547  \\ 
 cti & 	 318 & 	 \textbf{318} & 	 \textbf{916} & 	 917 & 	 1716 & 	 \textbf{1716} & 	 \textbf{2755} & 	 2778 & 	 \textbf{4089} & 	 4132 & 	 \textbf{5754} & 	 5763  \\ 
 memplus & 	 5355 & 	 \textbf{5355} & 	 \textbf{9367} & 	 9418 & 	 \textbf{11626} & 	 11628 & 	 \textbf{13128} & 	 13130 & 	 \textbf{14248} & 	 14264 & 	 \textbf{16321} & 	 16724  \\ 
 cs4 & 	 361 & 	 \textbf{361} & 	 936 & 	 \textbf{936} & 	 1467 & 	 \textbf{1467} & 	 \textbf{2099} & 	 2126 & 	 \textbf{3009} & 	 3014 & 	 \textbf{4097} & 	 4107  \\ 
 bcsstk31 & 	 2676 & 	 \textbf{2676} & 	 \textbf{7176} & 	 7181 & 	 \textbf{13234} & 	 13246 & 	 \textbf{23321} & 	 23504 & 	 \textbf{37311} & 	 37459 & 	 \textbf{58319} & 	 58667  \\ 
 fepwt & 	 340 & 	 \textbf{340} & 	 704 & 	 \textbf{704} & 	 \textbf{1414} & 	 1416 & 	 \textbf{2781} & 	 2784 & 	 \textbf{5587} & 	 5606 & 	 \textbf{8312} & 	 8346  \\ 
 bcsstk32 & 	 4667 & 	 \textbf{4667} & 	 8778 & 	 \textbf{8778} & 	 \textbf{20013} & 	 20035 & 	 \textbf{35635} & 	 35788 & 	 \textbf{59321} & 	 59824 & 	 \textbf{91772} & 	 92690  \\ 
 febody & 	 262 & 	 \textbf{262} & 	 598 & 	 \textbf{598} & 	 \textbf{1032} & 	 1033 & 	 \textbf{1755} & 	 1767 & 	 \textbf{2874} & 	 2906 & 	 \textbf{4878} & 	 4982  \\ 
 t60k & 	 71 & 	 \textbf{71} & 	 207 & 	 \textbf{207} & 	 454 & 	 \textbf{454} & 	 \textbf{819} & 	 822 & 	 \textbf{1386} & 	 1391 & 	 \textbf{2182} & 	 2198  \\ 
 wing & 	 774 & 	 \textbf{774} & 	 \textbf{1633} & 	 1636 & 	 \textbf{2502} & 	 2551 & 	 \textbf{3926} & 	 4015 & 	 \textbf{5824} & 	 5832 & 	 \textbf{8007} & 	 8043  \\ 
 brack2 & 	 684 & 	 \textbf{684} & 	 \textbf{2834} & 	 2839 & 	 \textbf{6896} & 	 6980 & 	 \textbf{11562} & 	 11622 & 	 \textbf{17370} & 	 17491 & 	 \textbf{26052} & 	 26366  \\ 
 finan512 & 	 162 & 	 \textbf{162} & 	 324 & 	 \textbf{324} & 	 648 & 	 \textbf{648} & 	 1296 & 	 \textbf{1296} & 	 2592 & 	 \textbf{2592} & 	 10560 & 	 \textbf{10560}  \\ 
 fetooth & 	 \textbf{3790} & 	 3792 & 	 \textbf{6826} & 	 6862 & 	 \textbf{11393} & 	 11422 & 	 \textbf{17500} & 	 17655 & 	 \textbf{25512} & 	 25624 & 	 \textbf{35501} & 	 35830  \\ 
 ferotor & 	 1960 & 	 \textbf{1960} & 	 \textbf{7100} & 	 7182 & 	 \textbf{12506} & 	 12546 & 	 \textbf{20169} & 	 20356 & 	 \textbf{31440} & 	 31763 & 	 \textbf{46382} & 	 47049  \\ 
 598a & 	 2367 & 	 \textbf{2367} & 	 \textbf{7863} & 	 7873 & 	 \textbf{15749} & 	 15820 & 	 \textbf{25758} & 	 25927 & 	 \textbf{39299} & 	 39525 & 	 \textbf{57599} & 	 58101  \\ 
 feocean & 	 311 & 	 \textbf{311} & 	 \textbf{1696} & 	 1698 & 	 \textbf{3963} & 	 3974 & 	 \textbf{7797} & 	 7838 & 	 \textbf{12575} & 	 12746 & 	 \textbf{20669} & 	 21033  \\ 
 144 & 	 6438 & 	 \textbf{6438} & 	 \textbf{15104} & 	 15122 & 	 \textbf{25257} & 	 25301 & 	 \textbf{37665} & 	 37899 & 	 \textbf{56205} & 	 56463 & 	 \textbf{80057} & 	 80621  \\ 
 wave & 	 \textbf{8615} & 	 8616 & 	 \textbf{16787} & 	 16822 & 	 \textbf{28613} & 	 28664 & 	 \textbf{42483} & 	 42620 & 	 \textbf{61983} & 	 62281 & 	 \textbf{85859} & 	 86663  \\ 
 m14b & 	 3823 & 	 \textbf{3823} & 	 \textbf{12964} & 	 12977 & 	 \textbf{25485} & 	 25550 & 	 \textbf{41939} & 	 42061 & 	 \textbf{65638} & 	 65879 & 	 \textbf{99467} & 	 100064  \\ 
 auto & 	 \textbf{9685} & 	 9716 & 	 \textbf{25922} & 	 25979 & 	 \textbf{44942} & 	 45109 & 	 \textbf{75719} & 	 76016 & 	 \textbf{120086} & 	 120534 & 	 \textbf{171640} & 	 172357  \\ 
 \hline

\end{tabular}
 \end{center} \caption{Improveing existing partitions $\epsilon = 3$\%}
\end{table}
\end{landscape}


==> tables/walshaw-improve-KaFFPa-eps-5.tex <==
\begin{landscape}
\begin{table}[H]
\begin{center}
\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|}\hline

 Graph  & \multicolumn{2}{|c|}{2} & \multicolumn{2}{|c|}{4} & \multicolumn{2}{|c|}{8} & \multicolumn{2}{|c|}{16} & \multicolumn{2}{|c|}{32} & \multicolumn{2}{|c|}{64}\\

\hline 
\input{tables/raw_tex_data_improve_5.tex} 
\hline

\end{tabular}
 \end{center} \caption{Improveing existing partitions $\epsilon = 5$\%.}
\end{table}
\end{landscape}

